Double parton distributions in the nucleon from lattice QCD

We evaluate nucleon four-point functions in the framework of lattice QCD in order to extract the first Mellin moment of double parton distributions (DPDs) in the unpolarized proton. In this first study, we employ an nf = 2 + 1 ensemble with pseudoscalar masses of mpi = 355 MeV and mK = 441 MeV. The results are converted to the scale mu = 2 GeV. Our calculation includes all Wick contractions, and for almost all of them a good statistical signal is obtained. We analyze the dependence of the DPD Mellin moments on the quark flavor and the quark polarization. Furthermore, the validity of frequently used factorization assumptions is investigated.

==> tables/FF_p2_fit.tex <==
\begin{tabular}{c|ccc|c}
\hline
\hline
form factor & $F(0)$ & $M^2[\mathrm{GeV}^2]$ & $p$(fixed) & $\chi^2/\mathrm{dof}$\\ 
\hline
$F_1^u$ & $2.003(13)$ & $1.063(19)$ & $2$ & $1.09$ \\
$F_2^u$ & $1.787(38)$ & $0.982(44)$ & $2$ & $1.63$ \\
$F_1^d$ & $1.0558(71)$ & $0.766(13)$ & $2$ & $7.15$ \\
$F_2^d$ & $-1.767(23)$ & $0.834(19)$ & $2$ & $2.51$ \\
\hline
$g_A^u$ & $0.9045(82)$ & $1.971(64)$ & $2$ & $1.61$ \\
$g_P^u$ & $29.99(95)$ & $0.327(11)$ & $2$ & $0.30$ \\
$g_A^d$ & $-0.2945(42)$ & $1.800(81)$ & $2$ & $1.05$ \\
$g_P^d$ & $-9.66(78)$ & $0.305(27)$ & $2$ & $0.13$ \\
\hline
\hline
\end{tabular}


==> tables/FF_p3_fit.tex <==
\begin{tabular}{c|ccc|c}
\hline
\hline
form factor & $F(0)$ & $M^2[\mathrm{GeV}^2]$ & $p$(fixed) & $\chi^2/\mathrm{dof}$\\ 
\hline
$F_1^u$ & $1.961(12)$ & $1.747(29)$ & $3$ & $1.79$ \\
$F_2^u$ & $1.733(35)$ & $1.674(68)$ & $3$ & $0.52$ \\
$F_1^d$ & $1.0167(61)$ & $1.300(19)$ & $3$ & $2.06$ \\
$F_2^d$ & $-1.680(20)$ & $1.456(29)$ & $3$ & $1.30$ \\
\hline
$g_A^u$ & $0.8965(79)$ & $3.161(97)$ & $3$ & $0.82$ \\
$g_P^u$ & $24.85(63)$ & $0.688(17)$ & $3$ & $1.03$ \\
$g_A^d$ & $-0.2910(39)$ & $2.90(12)$ & $3$ & $0.93$ \\
$g_P^d$ & $-7.92(49)$ & $0.638(44)$ & $3$ & $0.60$ \\
\hline
\hline
\end{tabular}

